LTL Model-Checking for Dynamic Pushdown Networks Communicating via Locks

A Dynamic Pushdown Network (DPN) is a set of pushdown systems (PDSs) where each process can dynamically create new instances of PDSs. DPNs are a natural model of multi-threaded programs with (possibly recursive) procedure calls and thread creation. Extending DPNs with locks allows processes to synchronize with each other. Thus, DPNs with locks are a well adapted formalism to model multi-threaded programs that synchronize via locks. Therefore, it is important to have model-checking algorithms for DPNs with locks. We consider in this work model-checking for DPNs with locks against single-indexed LTL properties of the form V fi s.t. fi is a LTL formula interpreted over the PDS i. We consider the model-checking problems w.r.t. simple valuations (i.e, whether a configuration satisfies an atomic proposition depends only on its control location and held locks) and w.r.t. regular valuations (i.e., the set of the configurations satisfying an atomic proposition is a regular set of configurations). We show that these model-checking problems are decidable.

==> relatedwork.tex <==
\section{Related work}
{\bf CTPL}: In \cite{CGB86,BCG89}, E.M. Clarke et al extended CTL
logic with index variables (ICTL) which range over processes, and
applied to reasoning about networks of identical processes. The
index variables is introduced to distinguish between the atomic
propositions of the different processes. Wolper also proposed a
logic (IPTL) for reasoning about data-independent programs, i.e.,
single reactive non-terminating program, similar to ICTL
\cite{Wol86} other than index variables are range over data
elements. In some sense, ICTL (resp. IPTL) is similar to CTPL when
only one variable whose domain is process ids (resp. date domain) is
permitted in each atomic proposition.

Later, A. P. Sistla et al extended CTL logic to COUNT CTL (CCTL)
\cite{SWZ07} for specifying properties of concurrent programs, which
is more expressive than the ICTL logic of \cite{CGB86,BCG89}. The
COUNT operator is used to count the number of process of a set of
process ids such that the process satisfies the specified property.
The model checking is carried out on the quotient structure
constructed from a reachability graph based on labelling algorithm.
To compare with CCTL, CTPL can express over only universal or
existential of process ids.

In \cite{BDGHL98}, J. Bohn et al proposed a first order CTL (FO-CTL)
model checking algorithm for first order Kripke structure. It
iteratively computes valuations for each node of the product
structure, the product of first order Kripke structure and a tableau
corresponding to the formula, whereas it will not terminate if the
data domain is infinite. Obviously, FO-CTL has more expressive power
than CTPL.

Much effort has been put into formula language extension of CTL in
some form. S. Roch presented an extension of the CTL, eCTL, offers
facilities for the limitation of the range of quantifiers in
temporal operators using transition formulae \cite{Roc00}. Model
checking eCTL for finite systems is easily implemented based on
work-list algorithm or symbolic algorithm, i.e, BDD-based algorithm.
The expressive power of eCTL is more than CTL, but less than the
modal $\mu$-calculus. \cite{BDL98,BSEFGR01} proposed the RCTL logic
using deterministic $\omega$-automata connectives which has more
expressive power than CTL. \cite{BDL98} also has shown a on-the-fly
model checking algorithm for finite automata based on translating
RCTL formulas into CTL formulas and appropriate finite automata, and
using CTL model checking algorithms. T. Br{\'a}zdil and I. Cern{\'a}
generalized the RCTL logic (RegCTL) by indexed the until operator
with a regular expression so that it is more expressive power than
either CTL or RCTL \cite{BC06}. The RetCTL model checking for finite
systems can be carried out using automatic-theoretic algorithm,
i.e., reduction of the model checking problem to the nonemptiness
problem of the product automata. R. Mateescu et al presented an
extension of CTL with regular expression (CTRL) where each temporal
operator except until operator is indexed by an regular formula
\cite{MMDJ08}. Although the until operator is not indexed by an
regular formula, the until operator indexed by an regular formula
can be expressed using \textbf{EF} operator. Thus the CTRL logic
subsumes RegCTL and eCTL. Recently, in \cite{AHKLL10,AHKLL10-full}
Roland Axelsson et al introduced a generic extension of CTL which
refines the until and release operators with formula languages,
i.e., regular languages, context-free languages. The formula
languages are characterized by $\tau$-finite automata,
$\tau$-visibly pushdown automata, $\tau$-pushdown automata where
$\tau$ is either deterministic or non-deterministic, in order
measure the complexity estimations. The model checking problem for
these logic are argued for both finite transition systems and
infinite transition system represented by visibly pushdown systems.
Each extension of the CTL logic refines the path of the transition
systems, while CTPL introduces variables into atomic propositions
and has same expressive power as CTL when the domain is finite. Thus
CTPL logic are incomparable with these logic, and is included in
these logic when the domain is finite.

J. Kinder et al introduced the CTPL logic used to describe program
behavior, i.e., behavior of malicious code and computer worm
\cite{KKSV05,KKV10}. In \cite{KKSV05,KKV10}, program is regarded as
a Kripke structure, and malicious behavior is specified in term of
CTPL as properties w.r.t Kripke structure. Consequentially, viruses
are detected using model checking technique. Although the logic used
in this paper is analogue of \cite{KKSV05,KKV10}, the model for our
model checking are PDSs which are well adapted to model programs
with (recursive) procedure calls.

